Evaluating Large Language Models for Generalization and Robustness via Data Compression

Existing methods for evaluating large language models face challenges such as data contamination, sensitivity to prompts, and the high cost of benchmark creation. To address this, we propose a lossless data compression based evaluation approach that tests how models' predictive abilities generalize after their training cutoff. Specifically, we collect comprehensive test data spanning 83 months from 2017 to 2023 and split the data into training and testing periods according to models' training data cutoff. We measure: 1) the compression performance on the testing period as a measure of generalization on unseen data; and 2) the performance gap between the training and testing period as a measure of robustness. Our experiments test 14 representative large language models with various sizes on sources including Wikipedia, news articles, code, arXiv papers, and multi-modal data. We find that the compression rate of many models reduces significantly after their cutoff date, but models such as Mistral and Llama-2 demonstrate a good balance between performance and robustness. Results also suggest that models struggle to generalize on news and code data, but work especially well on arXiv papers. We also find the context size and tokenization implementation have a big impact of on the overall compression performance.

==> bp.tex <==
According to equation \ref{source_coding} and \ref{chain_rule}, the theoretical minimum length (in bits) required to encode \(X\) with \(f\) is as follow:
\begin{equation}
    L(x_{1:n}) = -\sum_{i=1}^n\log P(x_i|x_{1:i-1})
\end{equation}
However, due to modern Transformer-based language models has a limited context window denoted as \(C\), we need to segment the dataset \(X\) into chunks of size \(C\) and feed them to language models one-by-one. As a result, the minimum length to encode \(X\) turns to:
\begin{equation}
    L(x_{1:n}) = -\sum^N\sum_{j=1}^C \log P(x_j|x_{1:j-1})
    \label{batch compression}
\end{equation}
where \(N\) represents the number of chunks. According to \(L(x_{1:n})\), we have the two major metrics for textual data compression: Bits per Token (BPT) and Bits per Character (BPC). BPC is defined as \(L(x_{1:n})\) divided by number of character in \(X\). In contrast, BPT is defined as \(BPT = L(x_{1:n})/n\) where \(n\) is the number of tokens. To review the compression procedure in character level, the tokenisation can be viewed as a pre-compression, as modern language model is often work on subwords. BPT, unlike BPC, aims to compare models' actual prediction capability in token level, which means it would not consider the efficiency of tokenisation process. BPC, on the contrary, takes both tokenisation and prediction into consideration where tokenisation can be viewed as a pre-compression.

It is rather straightforward to further apply language model to compress multi-modality data. In this setting, our dataset to compress consists a stream of bytes instead of tokens. In real practice, each byte was represented as an integer ranging from 0-255 and was fed to language model as a token. Similar to textual data, we chunk the byte streams into batches to feed to language models. And got the theoretical minimum length \(L(x_{1:n})\) required to encode \(X\), where differently \(x\) represents a byte instead of a token for multi-modality data. As here the model works directly on bytes stream, we use Bits per Byte (BPB) as the metric measuring compression performance. 

Note that, BPT, BPC, and BPB are all targeting on the theoretical minimum length to encode the data, so there is no physical compression conducted. We use this these metrics for the comparison among different language models as they are more straightforward. But to compare the compression ratios of language models to classic compression algorithms, e.g., gzip and FLAC, we need to utilise an entropy encoder to further finish the compression. Here we choose arithmetic coding since it is well-known for its optimal coding length. The actual compression process with language model and arithmetic coding and decoding are shown in Algorithm \ref{Arithmetic Coding} and \ref{Arithmetic Decoding}. Note that the language model is working on chunks, the arithmetic coding is also performed on chunked batches and then the compressed data are concatenated to be the final results.

We use compression ratio to benchmark compression algorithms, which is defined as the size of raw compressed data divided by size of the original raw data. Note that classical compressors often include a header or footer in their compressed output, here we do not consider the cost of these part in compression ratio computing.

=====

\subsection{Compression and Prediction}

It is well established that compression is essentially prediction. The source coding theory from Shannon's information theory \cite{shannon1948mathematical} suggests that the number of bits required by an optimal entropy encoder to compress a message is equal to the negative \(\log_2\) likelihood of the message given by a statistical model. In other words, minimising the negative \(\log_2\) likelihood of the message according to the statistical model is equivalent to minimising the bits required after compression. Formally, consider a stream of symbols \(x_{1:n}\), the optimal number of bits required to encode this stream is given by the formula:
\begin{equation}
L(x_{1:n}) = -\log_2 \hat P(x_{1:n}) = - \sum_{t=1}^n \log_2 \hat P(x_t|x_{1:t-1})
\label{source_coding}
\end{equation}

where \(L\) is the length to encode \(x_{1:t}\) in bits; \(P(x_{1:t})\) is the likelihood of \(x_{1:t}\) given the statistical model, followed by its expansion with the familiar chain rule:
\begin{equation}
    \hat P(x_{1:n}) = \prod^n_{i=1} \hat P(x_i|x_{1:i-1})
    \label{chain_rule}
\end{equation}
Considering the language modelling objective we use in language model pre-training is \(-\sum_{t=1}^n \log \hat P(x_t|x_{1:t-1})\), the same as Eq.~\ref{source_coding}, therefore we see that optimising the language modelling objective is fundamentally optimising the expected message length to compress \(x_{1:n}\). So stronger language modelling capability leads to better compression performance and verse versa.

In fact, compression prediction equivalence holds universally, not just in language modelling. Consider a universal compressor \(c\) on all computable distributions, its encoding length for \(x_{1:n}\) is denoted as \(l_c(x_{1:n})\). We have the following inequality based on Kolmogorov complexity \cite{kolmogorov1963tables,li2008introduction}:
\begin{equation}
    K(x_{1:n}) \leq |l_c(x_{1:n})| + K(c) + O(1)
\end{equation}
where \(K(x_{1:n})\) is defined as the length of the shortest possible description that produces \(x_{1:n}\) when run on a fixed reference universal Turing machine. This indicates an optimal lower bound for the compression algorithm. We also consider the Solomonoff predictor~\cite{rj1964formal} as a Bayesian mixture of all predictors that can be programmed in a chosen Turing-complete programming language. It is considered to be universally optimal for prediction,
\begin{equation}
    S(x_{1:n})=\sum_{q\in Q} 2^{-K(q)}q(x_{1:n})
\end{equation}
where \(S(x_{1:n})\) is the probability of \(x_{1:n}\) given by the Solomonoff predictor, which is equal to the distribution from all possible predictors \(q\) weighted by their simplicity (the shortest possible description of the predictor, i.e., Kolmogorov complexity of \(q\)); \(Q\) is the set of all predictors that can be programmed and computed. Therefore, for an individual predictor \(q\), we have the following inequality:
\begin{align}
    S(x_{1:n}) & \geq 2^{-K(q)}q(x_{1:n}) \\
    -\log_2 S(x_{1:n}) & \leq -\log_2 q(x_{1:n}) + K(q) + O(1) \label{solomonoff}
\end{align}
Comparing Eqs.~\ref{solomonoff} to \ref{source_coding}, as both \(K(c)\) and \(K(q)\) are constant and independent of the sequence length, we find compressing optimally is equivalent to predicting optimally and vice versa \cite{hutter2004universal,deletang2023language}. As a result, information compression can serve as a direct measure for both language models and universal predictor.

On the other hand, compressors can also serve as predictors \cite{deletang2023language}. A compressor \(c\)  can always sample the next byte from the following distribution:
\begin{equation}
    \hat P(x_i | x_{<i}) \sim 2^{l_c(x_{1:i-1}) - l_c(x_{1:i})}
\end{equation}
where \(l_c(x_{1:i})\) indicates the compressed length of \(x_{1:i}\) using compressor \(c\). This distribution means that if adding a particular byte \(x_i\) to the sequence \(x_{1:i-1}\) results in a relatively shorter compressed sequence, then \(x_i\) is more likely to be the correct next byte.

\subsection{Compression and Generalisation}

In the context of machine learning, \textcolor{orange}{the ability to compress information is often considered critical for the generalisation abilities}. For example, \citet{Hutter2006prize} argue that text compression and AI are equivalent problems, and thus introduce the large text compression benchmark, enwik9, which consists of the first \(10^9\) bytes of the XML text dump of the English version of Wikipedia on March 3, 2006. This is widely used in benchmarking compression algorithms and language models \cite{radford2019language,Chiang2023ChatGPT}.
Hutter further argue that predicting which characters are most likely to occur next in a text sequence requires vast real-world knowledge. A text compressor must solve the same problem in order to assign the shortest codes to the most likely text sequences \cite{hutter2004universal}.

\citet{sutskever2023generalization} argue that even Kolmogorov complexity  \(K(Y)\), as the ultimate compressor on dataset \(Y\) is undecidable, running a neural network with a SGD optimiser on the dataset \(Y\) can be seen as a method to search and approximate the optimal compressor. Sutskever further propose the concept so called conditional Kolmogorov complexity described as follow, claiming that unsupervised learning is to search the compressor that approximate the conditional Kolmogorov complexity:
\begin{equation}
    K(Y|X) \leq |c(Y|X)| + K(c) + O(1)
\end{equation}
where \(K(Y|X)\) indicates the shortest possible encoding length of dataset \(Y\) given an unsupervised dataset \(X\); \(|c(Y|X)|\) is the compressed length of dataset \(Y\) with the help of unsupervised dataset \(X\) using compressor \(c\) approximated by the neural network.
